Biometric Backdoors: A Poisoning Attack Against Unsupervised Template Updating

In this work, we investigate the concept of biometric backdoors: a template poisoning attack on biometric systems that allows adversaries to stealthily and effortlessly impersonate users in the long-term by exploiting the template update procedure. We show that such attacks can be carried out even by attackers with physical limitations (no digital access to the sensor) and zero knowledge of training data (they know neither decision boundaries nor user template). Based on the adversaries' own templates, they craft several intermediate samples that incrementally bridge the distance between their own template and the legitimate user's. As these adversarial samples are added to the template, the attacker is eventually accepted alongside the legitimate user. To avoid detection, we design the attack to minimize the number of rejected samples. We design our method to cope with the weak assumptions for the attacker and we evaluate the effectiveness of this approach on state-of-the-art face recognition pipelines based on deep neural networks. We find that in scenarios where the deep network is known, adversaries can successfully carry out the attack over 70% of cases with less than ten injection attempts. Even in black-box scenarios, we find that exploiting the transferability of adversarial samples from surrogate models can lead to successful attacks in around 15% of cases. Finally, we design a poisoning detection technique that leverages the consistent directionality of template updates in feature space to discriminate between legitimate and malicious updates. We evaluate such a countermeasure with a set of intra-user variability factors which may present the same directionality characteristics, obtaining equal error rates for the detection between 7-14% and leading to over 99% of attacks being detected after only two sample injections.

==> sections/attackdesign.tex <==

\section{Attack Design}

\todo{Choosing the starting/target sample is part of methodolgoy}

\label{sec:attackdesign}
Using the assumptions made in the system and threat model, we first present the challenges in designing the attack, then we show how adversarial samples are generated, and finally how the poisoning attack works.

\subsection{Overview}

The concept behind the poisoning attack is that the adversary adds adversarial samples to the legitimate user template in order to change the decision boundary of the classifier.
Figure~\ref{fig:poisoning-example} shows a two-dimensional representation of how the attack works.
There are three categories of samples:
\begin{itemize}[leftmargin=0.5cm]
	\item \textit{user samples}: legitimate user samples;
	\item \textit{adversary samples}: samples coming from the biometric trait of the adversary;
	\item \textit{poisoning samples}: samples algorithmically crafted by the adversary (commonly referred to as ``adversarial samples'').
\end{itemize}
Figure~\ref{fig:poisoning-example} shows how the user and adversary samples are well separated in the feature space, due to the uniqueness of their biometric traits.
At enrolment, a one-class classifier learns the distribution of the user samples creating a boundary around it, shown by the darker blue area.
The classifier is able to correctly discriminate between adversary and user samples, rejecting the adversary in an impersonation attempt.

Knowing his own and the user samples distribution, the adversary crafts the poisoning samples accordingly.
As the self-update threshold is in place, the adversary must make sure that the crafted samples lie within the current accepted region (blue area), otherwise they would be rejected as anomalous.
By injecting in the template one poisoning sample at a time, the adversary shifts the decision boundary towards his own sample distribution.
With sufficient poisoning samples, the adversary will move the decision boundary enough so that his own samples will fall inside it, and can therefore impersonate the user with his own trait.

%In the following, we first outline the challenges of performing such an attack, then we detail how the poisoning samples are generated and how the poisoning attack works.

\subsection{Challenges}

\begin{figure}[t]
	\includegraphics[width=0.48\textwidth]{images/poisoning-example}
	\caption{Changes in the classifier decision boundary (dark blue line) with the addition to the template of adversarial crafted samples. With enough poisoning samples, the classifier will recognize the adversary as the legitimate user.}
	\label{fig:poisoning-example}
\end{figure}

%The poisoning attack is difficult for many reasons.
%In a zero-effort scenario, the adversary could inject his own samples simply by attempting impersonation with his own trait.
%In this case, the attack would work only when the two distributions of Figure~\ref{fig:poisoning-example} initially overlap.
%This means that the attack would be as successful as the system FAR, but would also make the poisoning unnecessary (the adversary can already impersonate the user).
The challenges are based on the limited injection capabilities and on the unknown location of the user template.

\todo{rephrase this for \# queries and capabilities limitations. Weak attacker comes from the fact that he can fail to inject}

\myparagraph{Embedding Space} Figure~\ref{fig:poisoning-example} shows a simplified 2-dimensional example of the user distribution.
This distribution is actually in an \textit{n}-dimensional embedding space (that consists of 128 or 256 dimensions for face and speaker recognition, respectively).
If the adversary had control over the location of samples in this space, he could simply craft and inject the poisoning samples that lie on the \textit{n}-dimensional vector between the user and adversary distribution centroid.
However, the adversary only controls the raw biometric measurements (images or sounds) and furthermore needs to deal with the noise that inevitably occurs with the biometric measurement.
It becomes therefore hard to find a direction between user and adversary samples in the embedding space, as this is incorporated whithin the DNN, which the adversary cannot alter.

\myparagraph{Unkown Training Data} Even when a direction is found, another important challenge remains for the weak attacker.
As he only has one user sample that is not part of the template, he has no information about the training data and consequently the decision boundary of the template update procedure (blue area in Figure~\ref{fig:poisoning-example}).
This is an extremely weak assumption, and it brings the following obstacle: the adversary does not know whether a crafted intermediate sample would be accepted by the system.
Every injection attempt by the weak adversary needs to be physically carried out: adversary crafts an intermediate sample, presents the sample to the system and monitors the outcome (i.e., sample was accepted or rejected).
Clearly, crafting intermediate samples and presenting the sample to the system are fairly expensive action for the weak attacker: he might raise suspicion and sample crafting might require resources.
Therefore, random (or plain iterative) approaches are not a good strategy for the poisoning, as at every attempt the risk of being detected and the cost of the attack grows.
Additionally, the system could also block the template updating procedure after repeated failed attempts.




\subsection{Adversarial Sample Generation}\label{sec:adv_sample_gen}
%The problem of generating adversarial samples is generally defined as follows: given a model,  an input sampleand a desired output class, the input sample
Generally, in order to generate adversarial samples, the attacker needs an initial sample, a DNN, and a desired network output class.
The adversary then iteratively perturbs the feature of the initial sample in order to shift its DNN output class towards the desired one.
The generation of adversarial samples in DNNs is generally based on solving an optimization problem on the network \textit{softmax} layer (the output layer, which indicates the classes probability). 
The presence of a softmax layer facilitates the problem definition: an adversarial sample should present feature perturbations which create an increment in the probability for the desired target class while decreasing the probabilities of other classes.
However, in our system model, the DNN does not output a softmax layer, but an embedding in a reduced multidimensional space.
In this case, focusing on a single class in the output layer is not sufficient, as we need to decrease the overall distance in the multi dimensional network output.
We therefore re-define the optimization problem in order to reduce the distance between the desired target output and the current sample output.

\myparagraph{Formulation}
Formally, given a deep model $M$, a sample from the adversary $\vec{x}$, a sample from the user $\vec{y}$ and their respective embeddings computed by the model $M(\vec{x})$ and $M(\vec{y})$, we want to find a perturbation on the input features $\delta_x $ that minimizes the following:
\begin{equation}\label{eq:generation}
 \arg\min_{\delta_{\vec{x}}} \norm{M(\vec{x} + \delta_{\vec{x}}) - M(\vec{y})}_1,
\end{equation}

where $\norm{\cdot}_1$ is the \textit{L}1 norm function.
To find the optimal perturbations, we use gradient descent.
We first compute the Jacobian matrix of the model:
\[
J_M = \left[\frac{\partial M_j}{\partial \vec{x}_i}\right]_{ij}.
\]
The Jacobian matrix describes the relationship between changes in the DNN input and their effect on the output layer. 
Additionally, we compute the desired direction of the changes $\vec{d}$ as:
\[
\vec{d} = [\sign(M(\vec{x})_j - M(\vec{y})_j)]_j,
\]
where the $\sign$ function returns $1$ when the difference is positive, and $-1$ otherwise.
Intuitively, $\vec{d}_j$ indicates whether the desired changes in output $j$ is an increment or a decrement.
Inspired by~\cite{Papernot2017}, we re-define a saliency map $S$ over the input features $i$ by computing a dot product as follows:
\[
S(\vec{x}, \vec{y})_i = \vec{d} \cdot \left[ \frac{\partial M_0}{\partial \vec{x}_i}, ..., \frac{\partial M_n}{\partial \vec{x}_i} \right].
\]

\begin{algorithm}[t]
	\caption{Poisoning Sample Generation: neural network $M$, adversary sample $\vec{x}$, user sample $\vec{y}$, perturbation delta $\theta$, max iterations $N$, template update acceptance function $f$.}\label{alg:generation}
	\begin{algorithmic}[1]
		\INPUT{$M, \vec{x}, \vec{y}, \theta, N, f$}
		\State $\vec{x}^* \gets \vec{x}$\Comment{$\vec{x}^*$ is the current poisoning sample}
		\State $j \gets 0$
		\While{$\text{\textbf{not}} \ f(\vec{x}^*) \ \text{\textbf{and}} \ j < N$}
		\State compute $S(\vec{x}^*, \vec{y})$
		\State $i_1\gets \arg\max_i S(\vec{x}^*, \vec{y})$ \Comment{find best features}
		\State $i_2\gets \arg\min_i S(\vec{x}^*, \vec{y})$
		\State $\vec{x}^*_{i_1} \gets \vec{x}^*_{i_1} + \theta$ \Comment{apply perturbations}
		\State $\vec{x}^*_{i_2} \gets \vec{x}^*_{i_2} - \theta$
		\State $j \gets j +1$
		\EndWhile
		\State \textbf{return} $\vec{x}^*$
	\end{algorithmic}
\end{algorithm}

When the sign of the direction $\vec{d}_j$ matches the sign of the gradient $\frac{\partial M_j}{\partial \vec{x}_i}$ (both positive or both negative), then this indicates that increasing feature $i$ decreases the difference between the current and desired $j$-th output, $M(\vec{x})_j - M(\vec{y})_j$.
On the other hand, when the signs are mismatched, then the opposite is true: decreasing feature $i$ decreases the difference between the current and desired $j$-th output.

Using the dot product ensures that $S_i$ accounts for the overall effect on the outputs.
In fact, a perturbation on input $i$ will affect several (if not all) outputs $j$.
By multiplying the $\vec{d}_j$ with the magnitude of their respective gradient $\frac{\partial M_j}{\partial \vec{x}_i}$ and taking the summation of individual products, we account for the complete effect on the output.
The content of $S_i$ indicates how effective perturbations of feature $i$ are in moving the network output in the desired direction.
If $S_i$ is positive, increasing feature $i$ will cause an overall distance reduction between the current and the desired output.
When $S_i$ is negative, decreasing feature $i$ will cause an overall distance reduction between the current and the desired output.

\myparagraph{Generation Algorithm}
Algorithm~\ref{alg:generation} shows the algorithm used for the poisoning sample generation.
The attack needs the following inputs: a sample from the adversary $\vec{x}$, a sample from the victim user $\vec{y}$, a DNN model $M$, and a template update acceptance function $f$.
The function $f$ takes a sample in input and returns \texttt{True} when the sample would be accepted by the template update procedure, \texttt{False} otherwise.
The algorithm iteratively refines the adversary sample $\vec{x}^*$ by computing the map $S(\vec{x}^*, \vec{y})$ at each iteration and perturbing the two best features $i_1, i_2$.
A delta $\theta$ is used to limit the magnitude of the perturbation.
The algorithm stops when the poisoning sample is accepted by the function $f$, or when it reaches the maximum number of iterations, returning the generated sample.

%In some cases the algorithm might not obtain an accepted sample in the set number of iterations $N$ (due to the gradient descent optimization).
%The algorithm therefore

\subsection{Perfect Attacker}

As the perfect attacker has access to the training data, he knows the location of the current decision boundary.
Additionally, he has perfect injection capabilities, so he can directly use Alg.~\ref{alg:generation} to craft the necessary poisoning samples with no restrictions.
The perfect attacker scenario assumes a very strong adversary which might be unrealistic. 
We include it in our analysis for two main reasons: to obtain an empirical best-case limit on the poisoning attack (that we use as a baseline) and to learn the dynamics of the poisoning attack that we can re-use for the imperfect attacker (see Section~\ref{sec:pibbc}).


Algorithm~\ref{alg:attack} shows the poisoning attack steps.
The attack needs the same inputs as Alg.~\ref{alg:generation}, with the addition of the classifier $C$ and the user template used for training $Y$.
The user template is composed of the embeddings of raw user samples computed by the network $M(\vec{y}_i)$.
According to the system model, we train the classifier with the training data to represent the enrolment phase.
The algorithm then crafts a poisoning sample $\vec{x}^*$ using Alg.~\ref{alg:generation}.
As soon as the sample is accepted by the template update function, it is added to the user template, and the classifier is trained again with the augmented training set.
If the poisoning sample is not accepted by the template update function at the end of the iterations, then the attack fails.
This might happen when the gradient descent optimization gets stuck in a local optima, which causes the generated sample $\vec{x}^*$ to not be sufficiently close to the user sample $\vec{y}$ in the embedding space.
Algorithm~\ref{alg:attack} runs until the adversary sample is accepted by the classifier's update function, that is when it enters the template.

\begin{algorithm}[t]
	\caption{Poisoning Attack: neural network $M$, adversary sample $\vec{x}$, user sample $\vec{y}$, perturbation delta $\theta$, max iterations $N$, user template $Y=\{M(\vec{y}_0), ..., M(\vec{y}_n )\}$, classifier $C$.}\label{alg:attack}
	\begin{algorithmic}[1]
		\INPUT{$M, \vec{x}, \vec{y}, \theta, N, C, Y$}
		\State $C$ is trained with $Y$
		\While{\text{\textbf{not}} $C$ accepts $M(\vec{x})$ }
		\State $\vec{x}^* \gets \text{gen}(M, \vec{x}, \vec{y}, \theta, N, C\text{.update})$ \Comment{Algorithm 1}
		\If{$C$ accepts $M(\vec{x}^*)$}
		\State $Y \gets Y + \{M(\vec{x}^*)\}$  \Comment{Add to training set}
		\State $C$ is re-trained with $Y$
		\Else
		\State \textbf{return} \texttt{False}
		\EndIf
		
		\EndWhile
		\State \textbf{return} \texttt{True}
	\end{algorithmic}
\end{algorithm}

\subsection{Weak Attacker}
\label{sec:pibbc}

In this case, the adversary is limited in both knowledge and injection capabilities.
To account for the limited injection capabilities, we introduce factors that enhance the physical realizability of the injection.
To account for the limited knowledge, we develop an injection heuristic that estimates whether a crafted poisoning sample would be accepted by the unknown classifier.

\myparagraph{Physical Realizability}
As we consider an adversary with physical input manipulation capabilities (see Section~\ref{sec:threatmodel}), we need to account for the noise that occurs with the biometric measurement.
We therefore introduce noise factors in the steps of Algorithm~\ref{alg:generation}.
For face recognition, inspired by Sharif et al.~\cite{Sharif2016}, we implement the injection with a glasses frame worn by the attacker.
The adversary arbitrarily perturbs the colour of the frame to generate the desired poisoning sample.
Additionally, we account for the other factors affecting the input samples mentioned in~\cite{Sharif2016}: \textit{perturbations' robustness} and \textit{perturbations' smoothness}.
We therefore randomize the position of the frame at each iteration of Algorithm~\ref{alg:generation} and we look for perturbations $\delta_{\vec{x}}$ that cause set of inputs to be misclassified and minimize total variation~\cite{Mahendran2015}.
It should be noted that, differently from~\cite{Sharif2016}, our aim is not impersonation.
Instead, we aim to control the position of an input sample in the embedding space in order to carry out the poisoning attack.
For face recognition, the procedure for the injection is the following: (i) the adversary crafts a glasses frame, (ii) he attempts to login into the system while wearing the glasses.

For speaker recognition, we consider that rather than arbitrarily change the input sound in the time or frequency domain, the adversary can only statically increase specific frequencies of the input signal.
This could be done by having a speaker that plays a constant sound at a fixed frequency next to the system microphone.
We therefore limit changes to increments of specific frequency bands between 6KHz and 8KHz.
For speaker recognition, the procedure for the injection is the following: (i) the adversary crafts an audio sample that plays the required frequencies, (ii) he attempts to login into the system by pronouncing a word and simultaneously playing the crafted audio sample with a speaker.

\begin{figure}[t]
	\includegraphics[width=0.45\textwidth]{images/heuristic_face2}
	\caption{Distribution of \textit{L}2 distance between poisoning and user sample $\norm{M(\vec{x}^*) - M(\vec{y})}_2$ and number of perturbations applied to the poisoning sample. Each data point correspond to the first sample accepted by the template update function over the iterations of Algorithm~\ref{alg:generation}.}
	\label{fig:heuristic_plot}
\end{figure}

 
\myparagraph{Injection Heuristic}
As the adversary does not have access to training data and template update function he cannot use Alg.~\ref{alg:attack}.
In fact, he does not know whether (at any point) the crafted sample would be accepted by the system (he does not have $Y$, $C$ nor $C$.update).
However, the adversary can attempt to access the system with a crafted sample and learn from the outcome.
%In practice this corresponds to the adversary crafting a poisoning sample and presenting it to the system, and checking whether the impersonation worked.
%One approach would be gradually increasing the number of perturbations of the input, and attempting after each perturbation to access the system.
%Nevertheless, the adversary wants to minimize the number of impersonation attempts, as these require him to physically access the system and to craft an appropriate sample to inject.
In order to minimize the number of injections we develop a \textit{heuristic} to estimate whether a crafted poisoning sample would be accepted.
We use population data: the adversary pre-emptively runs the poisoning attack on a set of users (excluding the victim) to collect information about the acceptance behaviour of crafted samples.
The heuristic is based on two factors known by the adversary: (i) the number of perturbations applied to the input sample ($j$ in Alg.~\ref{alg:generation}) and (ii) the \textit{L}2 distance between the poisoning sample and the single known user sample $\norm{M(\vec{x}^*) - M(\vec{y})}_2$.

In practice, the adversary runs the attack for a set of users in the population for which he has knowledge of the template.
In this process, he runs Alg.~\ref{alg:attack} and for each sample returned by Alg.~\ref{alg:generation} (Line 3 in Alg.~\ref{alg:attack}) he collects the \textit{L}2 distance and the number of perturbations applied to the sample.
With this information, he can find a ``sweet spot'' in the two-dimensional space that indicates the likelihood of the current poisoning sample $\vec{x}^*$ of being accepted by the template update function. 
Figure~\ref{fig:heuristic_plot} shows confidence interval ellipses around the distribution of the accepted samples on the known population (at 68, 86 and 95\% confidence), for the first and for the second successfully injected sample.

Using the data gathered from the population, the adversary now has access to a good estimator of sample acceptance. 
In particular, the closer the current poisoning sample $\vec{x}^*$ is to the center of the two-dimensional distribution, the most likely the sample will be accepted by an unseen template update function.
The adversary therefore uses the heuristic to decide which  $\vec{x}^*$ to inject.
If the injection fails (the poisoning sample cannot impersonate the user), he just fallbacks to an iterative approach, where he runs Alg.~\ref{alg:generation} for an additional number of steps (increasingly shifting the poisoning sample towards the user sample), and attempts the injection again.


==> sections/conclusion.tex <==
\section{conclusion}
\label{sec:conclusion}

\todo{insight about maximum matcher being crap}

\todo{insight about choosing the nu parameter appropriately}

In this paper, we have presented an effective template poisoning attack that allows the adversary to place a biometric backdoor.
We use population data to develop a heuristic for a minimal knowledge attack which reduces the number of failed injection attempts tenfold. %and can tailor this heuristic to the system's security settings (e.g., the maximum number of rejected samples).
We have demonstrated the attack's effectiveness against state-of-the-art face and speaker recognition.
In 50\% of cases, 10 samples are enough to place the backdoor for both face and speaker recognition.
The attack has minimal effect on the overall FAR and FRR (less than 4\% increase for each metric).

Compared to previous work, we assume a much weaker adversary to achieve these results.
Specifically, the attack can be performed at any point during the system's life time (i.e., there is no need to compromise training data or the enrolment phase).
We also assume an attacker with minimal knowledge, i.e., the attacker does not know the user template, training data or decision boundaries.
We model the practical challenges of physical sample presentation for both speaker and speaker recognition, further lowering the attacker's assumed capabilities.
These assumptions about the attacker and the popularity of template updating in research and deployed products highlight the severity of the attack.
We propose several practical countermeasures that mitigate the threat while still allowing template updating in an unsupervised manner.


\begin{comment}
Future work:
{\color{red} to be done}
\begin{itemize}
\item Include X\% of attacker's template, not just a single point (although this point can be chosen in a smart way to make this less problematic)
\item Practical demonstration (voice, specifically)
\item Reduce impact on FRR (e.g., by injecting every Xth sample in the vicinity of the legitimate user's template)
\end{itemize}

Why is our work important?
\begin{itemize}
\item raise awareness to this attack and make sure people act on it, including it in the threat model.
\item question deep models?
\end{itemize}
\end{comment}



==> sections/discussion.tex <==

\section{Countermeasures} 
\label{sec:countermeasures}
\todo{maybe rename this to discussion and have a countermeasure subsection}

\todo{in discussion discuss why template sanitization is retarded}

\todo{in countermeasure make a point for attack getting harder as the legitimate distance between users grows in embedding space (more samples)}

\todo{different window update policies to discard old samples}

There are two groups of intuitive countermeasures, protecting the sample injection at the sensor or securing the template update procedure. 

\subsection{Sample Injection Defenses}

\todo{this subsection might go entirely}

\myparagraph{Liveness Detection}
When the poisoning samples present non-human like characteristics, liveness detection (or, more generally, presentation attack detection) is a well-known approach to protect from poisoning attacks.
As an example, when adversarial samples for speaker recognition are reproduced through a speaker for the injection, the time-difference-of-arrival in phonemes captured by the system microphone can signal the injection attempt~\cite{Zhang2016}. 
It should be noted that the same does not apply for face recognition with injection based on glasses, as the adversary would  perform the injection himself (therefore would present liveness).

\myparagraph{Adversarial Sample Resilience}
One approach to defend against poisoning attacks to increase the difficulty of finding the desired adversarial samples.
As an example, in adversarial training~\cite{Papernot2016}, the training data includes adversarial samples specifically crafted to increase the model resilience against them at test time.
Another approach, known as gradient masking, attempts to hide the network gradient at training time, making the network robust to small perturbations in the input~\cite{Papernot2016}.
However, both approaches are fundamentally arms race, with new attacks attempting to circumvent the additional barriers. 
This may slow down the development of effective attacks but it is unlikely to solve the problem for sufficiently popular systems. 
This is evidenced by recent attacks on state-of-the-art recognition systems (see Section~\ref{sec:relatedwork}). 
\subsection{Securing Template Updates}
\myparagraph{Second Factor Authentication} Requesting explicit authorization can be required before any new samples are added to the user template. 
This approach is already adopted by some systems (such as Windows Hello) but not used universally. 
Requiring explicit confirmation somewhat impacts the user experience, especially if the system would normally make frequent small updates (such as gradual lighting changes). 
In addition, this approach does not safeguard the user from adversaries that temporarily obtain the second factor necessary for the update (e.g., a password/PIN could be on a weekly change policy, which would give the adversary enough time to implant the backdoor). 

\myparagraph{Monitoring Update Behavior} Analysing the changes in template update habits could produce evidence of suspicious activity (such as sudden, frequent updates of the template). 
Biggio et al. propose a similar approach called ``template sanitization''~\cite{biggio2015adversarial}.
This approach is based around detecting subsequent template updates in a specific direction in feature space, arguing that legitimate updates would be more random in nature.
The approach might not be directly applicable when the direction is based on gradient descent and not statically pre-defined, but could be extended to allow some tolerance to direction changes.

If a suspicious update pattern is detected, future template updates could either be blocked completely or made subject to explicit second factor authorization (see above). 
In addition, both the time and content of template updates can be logged for review and evidence purposes. 
Logging would allow both manual inspection and rolling back the changes without needing to re-enrol if an attack is detected.




==> sections/evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

\begin{figure*}[t]
	\centering
	\begin{subfigure}[b]{0.2\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/Clint_Eastwood}
		\caption%
		{{\small adversary.}}    
		\label{fig:original_face}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.2\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{images/Clint_Eastwood_1}
		\caption[]%
		{{\small perfect attacker.}}    
		\label{fig:adversary1_face}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.2\textwidth}   
		\centering 
		\includegraphics[width=\textwidth]{images/Clint_Eastwood_3}
		\caption[]%
		{{\small weak attacker.}}    
		\label{fig:adversary2_face}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.2\textwidth}   
		\centering 
		\includegraphics[width=\textwidth]{images/Gerhard_Schroeder_0074}
		\caption[]%
		{{\small victim.}}    
		\label{fig:target_face}
	\end{subfigure}
	\vskip\baselineskip
	
	\begin{subfigure}[b]{0.2\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/raw_adv_voice}
		\caption%
		{{\small adversary.}}    
		\label{fig:original_voice}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.2\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{images/raw_adv_wb_voice}
		\caption[]%
		{{\small perfect attacker.}}    
		\label{fig:adversary1_voice}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.2\textwidth}   
		\centering 
		\includegraphics[width=\textwidth]{images/raw_adv_bb_voice}
		\caption[]%
		{{\small weak attacker.}}    
		\label{fig:adversary2_voice}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.2\textwidth}   
		\centering 
		\includegraphics[width=\textwidth]{images/raw_usr_voice}
		\caption[]%
		{{\small victim.}}    
		\label{fig:target_voice}
	\end{subfigure}
	
	\caption
	{Showing the crafted poisoning samples. The first row shows the input samples for face recognition, while the second row shows the input samples for voice recognition (log filterbank energies of the signal~\cite{Variani2014}). The figure show the original adversary sample (Figure ~\ref{fig:original_face}, ~\ref{fig:original_voice}), a poisoning sample in the perfect attacker scenario (Figure~\ref{fig:adversary1_face},~\ref{fig:adversary1_voice}), a poisoning sample in the weak attacker scenario (Figure~\ref{fig:adversary2_face},~\ref{fig:adversary2_voice}) and the target victim's sample (Figure~\ref{fig:target_face},~\ref{fig:target_voice}).} 
	\label{fig:poisoning_samples}
\end{figure*}

\begin{figure*}[t]
	\centering
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/generation_plot_face}
		\caption%
		{{\small face recognition.}}    
		\label{fig:generation_plot_face}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.45\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{images/generation_plot_voice}
		\caption[]%
		{{\small speaker recognition.}}    
		\label{fig:generation_plot_voice}
	\end{subfigure}
	\caption
	{Distance between the poisoning sample embedding $M(\vec{x}^*)$ and the SVM decision boundary over the iterations of Alg.~\ref{alg:generation}. The dashed line shows the EER threshold. Shaded areas show the 95\% confidence intervals.}
	\label{fig:generation_plot}
\end{figure*}

\begin{figure*}[t]
	\centering
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/poisoning_plot_face}
		\caption%
		{{\small face recognition.}}    
		\label{fig:poisoning_plot_face}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.45\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{images/poisoning_plot_voice}
		\caption[]%
		{{\small speaker recognition.}}    
		\label{fig:poisoning_plot_voice}
	\end{subfigure}
	\caption
	{Fraction of accepted adversaries in relation to the number of attempted sample injections.}
	\label{fig:poisoning_plot}
\end{figure*}


In this section, we first show the performance of the poisoning samples generation, then we evaluate the effectiveness of the attack, and show the changes in error rates caused by the poisoning.

\myparagraph{Experiment Description}
To evaluate the attack's effectiveness, we pick three users from the datasets and use them as adversaries, attempting to attack the remaining users.
This way, we obtain  3x87 and 3x102 pairs for face and voice recognition, respectively.
For each user, we pre-emptively split his samples into training and test set, compute a system-wise EER with the split and set the self-update acceptance threshold at EER threshold (distance from the separating hyperplane of SVM).
As such, any sample that is accepted by the classifier is subsequently added to the updated template.
For the perfect attacker scenario we run Alg.~\ref{alg:attack} for each user sample $\vec{y}$ in the training set.
For the weak attacker scenario we pick one sample in the victim's test set and run 
Alg.~\ref{alg:attack} using the injection heuristic of Section~\ref{sec:pibbc} (learned from the remaining users).
The training set size was fixed at 10 samples for both face and voice recognition (images and utterances, respectively).
For speaker recognition, the utterances undergo a windowing process (according to~\cite{Variani2014}), so that the inputs to the DNN are Mel-frequency cepstral coefficients of stacked frames.
In this case, we aggregate the classifier decision over the set of frames, with majority voting.


\subsection{Generation of Poisoning Samples}

Figure~\ref{fig:poisoning_samples} shows some examples of poisoning samples.
As discussed previously, while the perfect attacker has complete freedom on the input domain (images or frequency bands at specific times, Figure~\ref{fig:adversary1_face},~\ref{fig:adversary1_voice}), the weak attacker is limited: he can only change the colour of the glasses and statically increase the content of specific frequency bands (Figure~\ref{fig:adversary2_face},~\ref{fig:adversary2_voice}).
Figure~\ref{fig:original_face},~\ref{fig:original_voice} and Figure~\ref{fig:target_face},~\ref{fig:target_voice} show the original adversary samples and the target victim's samples.

We report in Figure~\ref{fig:generation_plot} the results of the optimization of Section~\ref{sec:adv_sample_gen} with  Algorithm~\ref{alg:generation}.
Figure~\ref{fig:generation_plot} shows that the perfect attacker obtains samples within the EER boundary faster, due to the perfect input manipulation and the knowledge of training data.
The weak attacker also obtains accepted samples even in presence of the input noise, domain limitations and limited knowledge discussed in Section~\ref{sec:pibbc}.
We found that in few cases (less than 3\% of times in our experiment), gradient descent gets stuck into local optima before reaching the decision boundary.
In this case, the weak attacker does not known whether the optimization failed, and therefore the attack would fail.
To avoid this the adversary could run the optimization multiple times, adding some randomness in the search (e.g., starting from a different adversary sample).


\subsection{Attack Performance}

Figure~\ref{fig:poisoning_plot} shows the attack success rate with increasing injection attempts.
For the perfect attacker, all attempts are successful by definition as he knows the exact decision boundaries and samples are placed with zero error.
For the limited attacker, failed injections are included in the graph, as failed attempts cause identical effort (e.g., by printing the frames of glasses when attacking face recognition).
The results show that even for the weak attacker, 14 and 13 samples are enough to place the backdoor in 60\% of cases (adversary-user pairs), for face and speaker recognition respectively.
As one would expect, the attack is faster for the perfect attacker, with 4 injections being enough to achieve the same success rate.
Compared to previously published poisoning attacks on DNNs, this is a relatively high fraction of the training set size.
This is a result of having to bridge the distance between the user and the attacker samples in the embedding space, since we do not assume control over the initial training data or over the DNN development and training.

Occasionally, we found that the injection samples from the weak attacker increases the distance of the adversary sample from the boundary and the attack consequently fails (around 20\% of cases for both speaker and face recognition, shown in Figure~\ref{fig:poisoning_plot} by the curves not reaching 100\% success).
This happens when the single user sample known by the adversary is not sufficiently close to the current template.
In this case, the injection of a crafted sample might shift the hyperplane orientation in a direction that brings the adversary sample further away from the boundary.
This is a convenient property of using SVM over other simpler distance based measures (e.g., euclidean), that would not present this resilience.
The adversary could overcome these situations by obtaining more than one user sample, and combine them to achieve a better estimation of the template location.

\subsection{Heuristic Performance}

The injection heuristic described in Section~\ref{sec:pibbc} provided an accepted sample 88\% and 68\% of times, for face and speaker recognition respectively (reported in Table~\ref{tab:far-frr}).
We additionally analyze the relationship between attack success, number of total sample injection attempts and number of failed attempts for the attack on face recognition in Figure~\ref{fig:attempts_plot}.
The figure shows the results for three different injection methodology: a simple iterative approach, a conservative heuristic and an aggressive one (more details can be found in Appendix~\ref{sec:appendix_a}).
Intuitively, in a conservative heuristic the adversary decreases the distance between injected samples, in order to achieve a higher likelihood of acceptance.

At first, Figure~\ref{fig:attempts_plot} shows how both heuristics save dozens of failed attempts which are required in an iterative approach.
To achieve 50\% success rate, the adversary would need more than 100 attempts (most of which failures) in a simple iterative approach, while 10 attempts are sufficient while using the heuristic.
Additionally, the plot shows that the aggressive strategy grants similar success rate to the conservative one rate (Figure~\ref{fig:heuristic_comp1}), but produces a higher number of failed attempts (Figure~\ref{fig:heuristic_comp2}).
In fact, conservative strategy achieves a 10\% higher success rate with zero failed injections compared to the aggressive one.

In more secure systems failed authentication attempts could be logged or cause the system to lock or cause closer manual inspection.
For example, the iPhone's FaceID allows at most five failed authentication attempts before forcing the use of the backup PIN (which the attacker may not know).
The adversary should therefore tailor the injection heuristic based on the number of failed attempts, deciding to be more conservative when failed injections come at a greater cost.


%The reduced injection success rate for voice is explained by the additional variation caused by averaging over stacked frames (see Section~\ref{sec:systemmodel}).

%\textcolor{red}{Experiments to show a "number of injections needed" vs "fraction of failures" plot are currently running. We can use this to tailor the attack to the penalty the system places on failed attempts (e.g., the iPhone's max-five-attempts rule).}





\begin{figure*}[t]
	\centering
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/heuristic_comp1}
		\caption%
		{{\small total attempts.}}    
		\label{fig:heuristic_comp1}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.45\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{images/heuristic_comp2}
		\caption[]%
		{{\small failed attempts.}}    
		\label{fig:heuristic_comp2}
	\end{subfigure}
	\caption
	{Fraction of accepted adversaries in relation to the number of total failed injection attempts (Figure~\ref{fig:heuristic_comp2}) and to the number of total injection attempts (Figure~\ref{fig:heuristic_comp1}). Data shown for the attack on face recognition.}
	\label{fig:attempts_plot}
\end{figure*}

\subsection{Effect on Error Rates}
Table~\ref{tab:far-frr} shows how the attack affects the system's FAR and FRR.
For both modalities there is an increase in the FAR.
This is intuitive, as the attack has to increase the fraction of the feature space that is accepted by the classifier to incorporate the attacker's template.
Nevertheless, the increase is small enough to suggest that it does not significantly affect users other than the attacker, unless they happen to be extremely similar to the attacker.

While both modalities also show an increase in the FRR, this is particularly pronounced for face recognition. This is most likely a result of the different number of training data.
The more samples are injected into the system (as a percentage of initial training set size), the more likely it is for old training samples to be less important in the overall template.
While the increase in FRR is most likely small enough to go unnoticed, it would be feasible for the attacker to counteract this trend.
This could be achieved by not just injecting the required intermediate samples, but also placing forged samples at the edge of the legitimate user's template, to strengthen it.


\begin{table}[h]
	\centering
	\begin{tabular}{c|c|c|c|c|c}
		\toprule
		\multirow{2}{*}{\textbf{Trait}} & \textbf{FAR} & \textbf{FAR} & \textbf{FRR} & \textbf{FRR}  & \textbf{Heuristic} \\
		& \textbf{(pre)} & \textbf{(post)} & \textbf{(pre)} & \textbf{(post)}  & \textbf{Success} \\
		\midrule
		\textbf{Face} & 8.98 & 9.83 & 8.87 & 12.22 & 88.04\\
		\midrule
		\textbf{Voice} & 12.13 & 14.57 & 12.36 & 13.75 & 68.07\\
		\bottomrule
	\end{tabular}
	\caption{Changes in error rates after the poisoning attack is completed, and injection heuristic success (percentages).}
	\label{tab:far-frr}
\end{table}

\todo{Choosing SVM nu parameter}


==> sections/introduction.tex <==
\section{Introduction}

In recent years, biometric authentication has become one of the preferred ways to address burdens associated with passwords (e.g., re-use, inconvenient creation policies and bad memorability).
With a long history of research, face and fingerprint recognition are the most popular modalities and authentication systems based on them are currently delivered with consumer products.

While earlier research focused on the performance of these modalities under a zero-effort threat model, current trends in biometric systems are also prioritizing high protection of biometric templates.
Templates in fact represent sensitive user data, and their leak might compromise the secrecy of the biometric trait in a permanent way.
Different measures can be used to protect user templates: standard file encryption, template protection algorithms, secure elements, and distributed template storage.
Nowadays, most commercial biometric systems use any combinations of these protection measures.
As an example, both Apple's TouchID and FaceID perform template matching and store templates in the protected secure enclave, and the data never leaves the device\footnote{https://images.apple.com/business/docs/FaceID\_Security\_Guide.pdf}.

The attention dedicated to the protection of templates makes them less likely to being the target of adversaries, but renders the attack at the sensor a more viable attack vector.
Presentation attacks in particular have been investigated by the research community.
In these attacks, the adversary attempts to reproduce an artifact that resembles the legitimate user's biometric trait, and presents the artifact to the sensor.
As modern systems increasingly rely on machine learning (ML) techniques for the recognition, adversarial ML approaches become more relevant for the creation of artifacts that fool the recognition (\textit{evasion} attack).

%
As the user template is highly protected, changing it directly is not an option for the attacker.
However, an adversary can bypass the protection measures by exploiting the \textit{template update} procedure.
During template update, the system replaces or adds recent samples to the user template.
As most biometrics either exhibit inherent variability (e.g., through aging or physiological changes) or are subject to changes in environment (e.g., lighting and viewing angle), template update becomes a crucial process.
%In this paper, we focus on an adversary that injects adversarial samples into the system in order to \textit{poison} the user template. 

%Template update is becoming a standard operation in biometric systems, aimed at improving recognition.
Depending on the system, updating is either supervised or unsupervised.
Supervised updating means that additional guarantees in the user identity are required before the update (e.g., Windows Hello requires the users to re-input their PIN or password before template update).
From a usability perspective, unsupervised updating represents a more desirable choice, as it is a seamless approach that does not require additional user interaction.
In unsupervised scenarios, the confidence in the user identity can be strengthened with the introduction of a \textit{self-update} threshold: a new sample for the update is discarded if it does not match a confidence threshold (e.g., needs to be sufficiently similar to the current user template).
For example, FaceID automatically augments the user template after successful authentication if the quality of the match is above a threshold~\cite{faceidsecurityguide}.

By exploiting this template update procedure an attacker can  inject adversarial samples into the user template to carry out a \textit{template poisoning} attack.
In this attack, the adversary corrupts the recognition algorithm allowing himself to impersonate the user with his own biometric trait.
The poisoned template is hard to detect, and creates a backdoor for the adversary in the long-term (until the adversarial samples are removed).
However, the adversary needs to overcome three key challenges: (i) he has limited capabilities to inject samples, (ii) he has limited knowledge of the authentication system and the legitimate user's template, (iii) he must avoid degrading the legitimate user's experience to avoid generating suspicion.
We break down these challenges into concrete research questions as follows.


\myparagraph{Research Questions}
\begin{itemize}[leftmargin=0.6cm]
%	\item Is unsupervised template updating vulnerable to 	
	%\item Can adversaries exploit unsupervised template updating to create biometric backdoors through injected intermediate samples?
	\item How do different threat models (i.e., knowledge and injection capability) affect the poisoning attack speed and success rate?
	\item How does the implanted backdoor affect the overall error rates of the system for the attacked legitimate user?
	%\item To what extent does the attack affect normal system operation by increasing false accept and false reject rates?
	%\item How can system parameters be chosen to prevent template poisoning while still accounting for legitimate template drift?
\end{itemize}
%When adversaries are able to inject samples to the system, they might be able to corrupt the integrity of the stored victim template in a way that allows the adversaries themselves to authenticate as the legitimate user, this is known as \textit{template poisoning}. 
%Successful poisoning of templates creates a backdoor that can be used by the adversary to access the authentication system. 
%The poisoning is very hard to detect in an automatic way, and grants permanent future access to the adversary (unless the poisoned samples are removed entirely).

To answer these questions, we choose two biometric modalities for the analysis: face and speaker recognition.
Besides its uses in high-security settings (e.g., border control), face recognition is widely used in unsupervised environments, making it an obvious choice.
Most recently, speaker recognition is becoming particularly important with the rise of smart speakers like Google Home and Amazon Echo. 
Without speaker recognition, smart speakers are subject to accidental attacks (e.g., the speaker responding to a TV or radio ad~\cite{alexaTV}) or hidden voice commands~\cite{Carlini2016}.
Both modalities have inherent variablity caused by changes in environment, sensor position and user behavior.
In this paper, we present a methodology to carry out poisoning attacks on biometric systems based on deep ML pipelines.
We evaluate our attack on state-of-the-art systems for voice and speaker recognition, showing that the attack is feasible even for adversaries with limited knowledge and capabilities.
Finally, we discuss possible countermeasures to these attacks.

\myparagraph{Contributions}
The contributions of this paper are as follows:
\begin{itemize}[leftmargin=0.6cm]
	\item We propose a methodology to plant \textit{biometric backdoors} by poisoning the legitimate user's template, without assuming any knowledge of the user template. (\todo{don't phrase it like this but both knowledge/capabilities})
	\item We prove the attack's effectiveness on state-of-the-art face and speaker recognition systems.
	\item We discuss a set of practical countermeasures against template poisoning attacks.
\end{itemize}

The rest of the paper is organised as follows: Section~\ref{sec:relatedwork} describes the related work, Section~\ref{sec:threatmodel} outlines the threat model assumed in the paper. Section~\ref{sec:systemmodel} describes our system model. Section~\ref{sec:attackdesign} presents the template poisoning attack, the results are given in Section~\ref{sec:evaluation}. We provide a discussion of countermeasures in Section~\ref{sec:countermeasures} and conclude the paper in Section~\ref{sec:conclusion}.


==> sections/relatedworks.tex <==
\section{Related Work}
\label{sec:relatedwork}

In this section, we first give a brief background on biometric recognition, we then discuss attacks on biometric systems, and then given an overview of the existing work in poisoning attacks.

\subsection{Biometric Recognition}
Both research community and industry have shown significant interest in biometric recognition in recent years.
Oftentimes, recognition of biometric traits is proposed as an approach to mitigate the shortcomings of passwords (such as bad memorability, password reuse and easy to guess passwords).
Previous research has shown that most biometrics present inherent intra-user variability, both for physiological and behavioral traits.
In the following we will give a brief overview of face and speaker recognition systems, and how intra-user variability affects the system.

\myparagraph{Face Recognition}
Modern face recognition systems are based on deep convolutional neural networks (DNN), where the input image undergoes transformation over several layers (e.g., OpenFace~\cite{Baltrusaitis2018}, FaceNet~\cite{Schroff}, VGG-Face~\cite{Parkhi15}).
The advantage of physiological traits (such as face), lies in high permanence: faces remain mostly unchanged over an individual's lifetime, even considering ageing factors.
This allows for recognition of individuals over longer timeframes without frequent re-training.
%However, while the \textit{physical characteristic} changes slowly, its measurement captured by the sensor is subject to a number of factors.
%In particular, lightning conditions,  user's pose and camera distance have been shown to have an impact the recognition~\cite{Schroff}.
%To address this issue, modern face recognition systems perform an \textit{alignment} step before the image is fed into the network.
%This step attempts to adjust the input measurement to account for those factors, but only partially compensates for the introduced variability.

\myparagraph{Speaker Recognition}
%Differently from speech recognition (where algorithms understand what words the user is saying), in speaker recognition the algorithm attempts to determine the identity of the talking user.
There are two categories of speaker recognition: text-dependent and text-independent.
Intuitively, in the first case the recognition is tied to the words that are being said, while in the second the algorithm aims to recognize users independently on the uttered words.
In text-independent recognition, the system uses the physiological components of one's voice (e.g., shape and size of vocal chords), in text-dependent recognition there is behavioral component (linked to what the system requires the user to utter).
Similarly to face, speaker recognition presents good permanence of the underlying physiological characteristics of the voice during adult life.
%However, the measurement suffers from significant intra-user variability, that is due mainly to the context of measurement (e.g., background noise) and, in particular in the text-independent case, to the different features presented by different user's utterances.
Recently, DNN~\cite{Variani2014} models have outperformed more traditional systems based on \textit{i}-vector representations of speakers~\cite{Garcia-Romero2011}.

\myparagraph{Template Update}
The operation of updating the user template after enrolment is essential to add  tolerance to the user recognition.
In fact, biometric traits present significant intra-user variations: repeated measurements of the same biometric trait for the same user will present slight variations.
%These differences are well known in the literature, and are mainly due to what is known as the context of measurement~\cite{seberz2018}.
For face recognition, factors such as lightning conditions, user's pose and camera distance have been shown to have an impact the recognition~\cite{Schroff}.
Similarly, for speaker recognition, different words pronounced by the user will present different features (particularly in the text-independent case), while retaining an underlying intra-user similarity.


The procedure of updating the template is becoming increasingly popular, both in academic papers and deployed products.
Both Apple's FaceID~\cite{faceidsecurityguide} and TouchID~\cite{touchidsupportpage} perform template update procedures.
FaceID performs template updates either after a new sample is accepted, or when a rejected sample is followed promptly by a correctly entered backup passcode.
Windows Hello also offer an ``improve recognition'' feature, where new samples of the user's face are collected and added to the template to improve the performances. 

%\myparagraph{Physiological} These traits measure distinctive physical properties of humans, such as fingerprints, iris patterns or face geometry.
%The main advantage lies in high permanence (e.g., fingerprints remain largely unchanged over an individual's lifetime), which allows authentication and recognition of individuals over longer timeframes without frequent retraining.
%While the \textit{physical characteristic} changes slowly, its measurement captured by the sensor is subject to a number of factors.
%As an example, face recognition has been shown to be sensitive to changes in lighting conditions as well as viewing angle and distance to the camera~\cite{Schroff}.
%In modern face recognition systems the input image goes through a pre-processing \textit{alignment} step which attempts to compensate for the effect of lightning and user pose.
%Currently, most face recognition algorithms are based on deep neural networks (e.g., OpenFace~\cite{Baltrusaitis2018}, FaceNet~\cite{Schroff}, VGG-Face~\cite{Parkhi15}).
%
%\myparagraph{Behavioural} These traits capture distinctive behaviour, rather than physical characteristics.
%A popular approach is to harvest the distinctiveness of the users' interation with devices.
%As such, the authentication can occur implicitly in the background without a user's involvement or even knowledge (\textit{implicit} authentication). 
%
%Keystroke dynamics (i.e., distinctive typing patterns) are one of the oldest behavioural biometrics, dating back to 1980 when Gaines et al. authenticated users of typewriters~\cite{gaines1980authentication}. 
%Similarly, mouse movement patterns have been used as a behavioral biometric.
%Mouse data have been collected in lab studies, over the web~\cite{gamboa2004behavioral} and on subjects' own machines~\cite{nakkabi2010improving}.
%Collecting data on subject's machines (either locally or through websites) avoids artificial constraints on lab studies, but at the same time differences in hardware may introduce bias into the data~\cite{jorgensen2011mouse}.
%As such, the proposed classifier might distinguish hardware, rather than users.
%
%With touchscreen-based mobile devices becoming increasingly popular, researchers have explored touch dynamics as a biometric trait.
%Frank et al. were among the first to show touch dynamics's distinctiveness~\cite{frank2013touchalytics}.
%The authors achieve a 0\% EER for intra-session authentication and 4\% across sessions.
%These results show that touch dynamics, like other behavioural biometrics, exhibit changes over time that are not captured during a single enrolment session.
%
%Speaker recognition possesses both physiological (e.g., shape and size of vocal chords) and behavioral components.\textcolor{red}{extend this}

\subsection{Attacking Biometric Recognition}
The rising interest in biometric recognition has also led to increased efforts in attacking the resulting systems.
% There are two main classes of attacks: presentation attacks against physiological traits and mimicry attacks against behavioral traits. 
In presentation attacks, the adversary crafts an artefact of a user's biometric trait and presents it to the biometric sensor.
One of the best-known examples is a fake finger that can be made from a variety of materials, with latex being a popular choice.
Most notably, succesful attacks have been demonstrated against the iPhone's TouchID~\cite{CCCTouchID}. 
Face recognition suffers from a similar vulnerability, with early systems often being fooled with a simple photograph~\cite{boehm2013safe}.
As photos of individuals are easily accessible, particularly through the rise of social media, there has been considerable effort to thwart this type of attack.
One approach is the use of infrared cameras that allow the distinction between a paper printout and a live face~\cite{WinHello}.
3D cameras have been proposed to distinguish between flat objects (such as printouts or computer screens) and the 3D geometry of real faces.
However, 3D printing technology allows the relatively cheap fabrication of masks that escape detection~\cite{faceidbrokenbyvietnamese}.
Eberz et al.~\cite{eberz2017broken} demonstrate an attack against the Nymi Band, a wristband that uses ECG for user authentication.
After obtaining data from a variety of sources (e.g., fitness trackers or medical devices), they use a cheap audio player to create and inject a forged signal. 

Similarly, in mimicry attacks, adversaries attempt to imitate  legitimate human behavior.
These attacks can be either manual or automatic.
The former involves the attacker training themselves to adapt their behavior to match that of the victim.
Often, this training process is computer-assisted.
Tey et al.~\cite{tey2013can} demonstrate this for keystroke dynamics, with a system giving positive and negative feedback during the training phase.
%Another hardware-assisted approach is a treadmill attack on gait authentication~\cite{kumar2015treadmill}.
Automatic attacks avoid the high effort and cognitive load of manual attacks.
Serwadda et al.~\cite{serwadda2013kids} show an attack on touchscreen dynamics involving a robot carrying out swipes instead of a human. 

In most of these attacks, the main challenges are creating an artifact and evading the presentation attack detection mechanisms.
As a consequence, often presentation attack detection ends up in an arms race, where adversaries improve their attacks to circumvent evermore sophisticated measures.
In this work, we do not investigate presentation attacks directly.
Rather, we use them as a building block to carry out the poisoning attack, in particular for the injection of adversarial samples.



\subsection{Poisoning Attacks}

%In the past decade, adversarial machine learning has become a well established field of research.
%Barreno et al.~\cite{barreno2006can} where among the first to question the security of machine learning models, introducing an attack taxonomy and possible countermeasures.
Adversarial machine learning has become extremely relevant due to the wide-spread use of deep neural networks (DNN), which are prone to being fooled by purposefully crafted adversarial samples.
Adversarial ML attacks have been classified into two main categories: \textit{evasion} (\textit{inference-time}) attacks and \textit{poisoning} (\textit{training-time}) attacks~\cite{papernotsok2018}.
In the evasion attack, the adversary attempts to craft a sample that is classified as belonging to a desired output class.
In the poisoning attack, the adversary injects adversarial samples into the training data in order to maximize an objective function (typically to cause misclassifications at test time).
%Ideally, adversarial samples present limited or imperceptible perturbations in the input domain, in a way that makes them hard to detect by a human observer.

%Recently many adversarial ML attacks have been proven physically realizable.
Both face recognition and voice-based systems have been proven vulnerable to evasion attacks. 
Carlini et al.~\cite{DBLP:journals/corr/abs-1801-01944} performed an attack on speech-to-text, showing a methodology to a sound waveform similar to a given waveform, but that is transcribed by the system as any phrase chosen by the adversary.
In another example, Sharif et al.~\cite{Sharif2016} demonstrate the feasibility of evasion attack against state-of-the-art face recognition systems.
The authors show that by using a carefully crafted frame of glasses an adversary is able to both evade face detection and to impersonate arbitrary users of the systems.
%In this paper we instead focus on poisoning attacks, where an adversary aims to obtain long-term unsuspicious access to a system.

Poisoning attacks in DNN have also been investigated.
Works such as~\cite{Gu2017} and~\cite{Liu2018} investigate the concept of poisoned neural network, a network that achieves state-of-the-art performance on testing data but misbehaves on specific inputs, known by the adversary.
A preliminary analysis of poisoning attacks on biometric systems was proposed by Biggio et al.~\cite{10.1007/978-3-642-34166-3}.
The authors present a poisoning attack where an adversary injects a set of samples that gradually shifts the user template towards the biometric trait of the adversary, allowing him to impersonate the user.
%However, their threat model assumes perfect injection capabilities by the adversary, which is not realistic in practice, as an adversary with free injection at the biometric sensor has likely already compromised the system.
%Additionally, their work is based non state-of-the-art representation of templates (eigenfaces), which is greatly outperformed by modern systems.


In this paper, we build on the extensive body of related work outlined above to develop a novel template poisoning attack.
In practice, the proposed attack is composed of two stages: intermediate sample generation and injection into the system.
Both face and speaker recognition have been shown to be vulnerable to a variety of attacks (see above).
We use these insights to model the injection process, taking into account various limitations an attacker would face in practice.
While the concept of template poisoning has been proposed before (see~\cite{10.1007/978-3-642-34166-3}), our work differs in several aspects:
We consider an attacker that is not just limited in knowledge (we assume \textbf{no} knowledge or control over training data), but also in his injection capabilities.
As such, our work bridges the gap between a purely theoretical attack that assumes both extensive knowledge and direct access to the classifier (rather than just the physical sensor) and practice.
In addition, we assume a system model based on a DNN for dimensionality reduction and an SVM for classification, which reflects the current state of the art.

\todo{make a table, put \cite{Biggio2011}, \cite{Biggio2013}, \cite{garofalo2018fishy}}

\begin{table}[h]\small
	\centering
	\begin{tabular}{c|c|c|c|c|c|c|c|c}
		\toprule
		\thead{Work} & \rotatebox[origin=l]{90}{\thead{liveness detection}} & \rotatebox[origin=l]{90}{\thead{input noise}} &  \rotatebox[origin=l]{90}{\thead{unknown template}}  & \rotatebox[origin=l]{90}{\thead{face recognition}} & \rotatebox[origin=l]{90}{\thead{speaker recognition}} & \rotatebox[origin=l]{90}{\thead{state-of-the-art\\models}} & \rotatebox[origin=l]{90}{\thead{unknown model}} &
		\rotatebox[origin=l]{90}{\thead{victims can still \\  use the system}} \\
		\midrule
		Biggio et al.~\cite{Biggio2013} & \ding{55} & \ding{55} &  \ding{55}* & \checkmark & \ding{55} & \ding{55} & \checkmark & \ding{55} \\	
		\midrule
		Our & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \ding{55} & \checkmark \\			
		\bottomrule
	\end{tabular}
	\caption*{\small*knowledge of best-matching sample out of \todo{ put how many} several samples.}
	\caption{Comparison to previous work. }
	\label{tab:comparison}
\end{table}





==> sections/systemmodel.tex <==





\section{System Model}
\label{sec:systemmodel}
\subsection{Background}
\label{sec:systemmodel-overview}
Modern biometric recognition is separated in four phases: development, enrolment, recognition and an additional fourth phase, template updating.



\myparagraph{Development}
During development, a DNN is trained on a large labelled dataset of biometric measurements.
The objective of the DNN is to learn how to transform user samples in a reduced-dimensionality linearly separable hyperspace.
The transformed samples are known as \textit{embeddings}~\cite{Baltrusaitis2018} (or \textit{projections}~\cite{Variani2014}).
This pre-trained network is then deployed with the biometric system.

\myparagraph{Enrolment}
At enrolment, the user presents his biometric trait to the sensor.
One or more measurements are taken, processed and fed into the DNN.
The resulting embeddings are stored as the \textit{user biometric template}, and are used to train the template matching procedure.

\myparagraph{Recognition}
During the recognition phase, whenever the user presents his trait to the sensor, the system measures it, feeds it into the DNN, and attempts to match the resulting embedding with the known biometric template (e.g., with a threshold).
If the match occurs, the user is successfully authenticated.

\begin{figure}[t]
	\includegraphics[width=0.45\textwidth]{images/system-model}
	\caption{System model of biometric recognition.}
	\label{fig:system-model}
\end{figure}

\myparagraph{Motivation}
Training a DNN in development allows it to represent the samples in a more efficient lower dimensionality space, where simpler distance measures effectively separate users samples (e.g., Apple claims that their FaceID neural network is trained with over 1 billion face images~\cite{faceidsupportpage}).
The recognition procedure should enable authentication without
requiring samples from other users (``negative class samples'').
This is desirable from a deployment perspective, as the system does not have to be shipped with other users' samples to make up the negative class. 
Another benefit of using one-class matching procedures is that they avoid potential privacy concerns of shipping biometric traits from other users as part of the biometric system.
Additionally, previous work has shown that the selection of users for the negative class greatly impacts the system's error rates~\cite{Eberz2017}.
However, outside specific settings such as insider threats, the system would be unlikely to contain samples belonging to an possible attacker.


%\myparagraph{Template Update}
%The operation of updating the user template after enrolment is essential to add some level of tolerance to the user recognition.
%In fact, biometric traits present significant intra-user variations: repeated measurements of the same biometric trait for the same user will present slight variations.
%%These differences are well known in the literature, and are mainly due to what is known as the context of measurement~\cite{seberz2018}.
%As an example, for face recognition, different poses of the user with respect to the camera affect the resulting biometric measurement.
%Similarly, for voice recognition, different words pronounced by the user will present different features, while retaining an underlying intra-user similarity (due to the uniqueness of the user voice).
%
%
%Template updating is becoming increasingly popular, both in academic papers and deployed products.
%Both Apple's FaceID~\cite{faceidsecurityguide} and TouchID~\cite{touchidsupportpage} perform template update procedures.
%FaceID performs template updates either after a new sample is accepted, or when a rejected sample is followed promptly by a correctly entered backup passcode.
%Windows Hello also offer an ``improve recognition'' feature, where new samples of the user's face are collected and added to the template to improve the performances. 

\subsection{Design Choices}
\todo{considering three matchers}
We focus on two biometric modalities: face recognition and speaker recognition (in the text-independent case).
The reason for this choice is that both modalities are sufficiently established and their state-of-the-art methodology follows the phases described in Section~\ref{sec:systemmodel-overview}.

An illustration of the system model assumed for the remainder of the paper is given in Figure~\ref{fig:system-model}.
New raw samples are first processed by a DNN.
Following the dimensionality reduction performed by the DNN, we classify the samples using a one class Support Vector Machine (SVM).
With a one class SVM means only one user's samples are needed to generate a template.
Following from the threat model in the previous section, both attackers know the DNN used by the system, and the parameters of the SVM classifier.
%In addition, it avoids underestimating error rates depending on how the negative class is selected~\cite{Eberz2017}.

For the template update procedure, we choose to use self-update with a threshold based on the SVM threshold.
In other words, if a sample is accepted by the classifier it is subsequently added to the training set.
This choice is similar to the unsupervised update process used by Apple's FaceID, where newly obtained samples are added to the template if the match quality is sufficient~\cite{faceidsecurityguide}.
Following the addition of a new sample, the classifier is then retrained.

The recognition systems we use are OpenFace~\cite{Baltrusaitis2018} and the methodology of Variani et al.~\cite{Variani2014}, for face and speaker recognition, respectively.
OpenFace offers the possibility to download the pre-trained DNN from their website, while for~\cite{Variani2014} we implement and train the DNN on our voice dataset.

\myparagraph{Datasets}
The datasets used in the analysis are reported in Table~\ref{tab:datasets}.
We selected these datasets because they have a significant number of samples per user and display sufficient intra-user variability.
In the case of face recognition, the main causes of variations are user pose and illumination.
For the~\cite{Huang2007} and~\cite{speechcommandsdataset} datasets we only retain users that have at least 20 samples.
For the voice datasets, the main causes of variations is the environment of recording and the utterance pronounced by the user.

\begin{table}[t]
	\centering
	\begin{tabular}{c|l|l|l}
		\toprule
		\textbf{Name} & \textbf{Trait}& \textbf{N}& \textbf{user samples} \\
		\midrule
		Extended Yale B~\cite{Lee2005} & face & 28 & >218 \\		
		\midrule
		Labeled Faces in the Wild~\cite{Huang2007} & face & 62 & >20 \\
		\midrule
		Speech Commands~\cite{speechcommandsdataset} & voice & 75 & >30 \\		
		\midrule
		VoxForge~\cite{voxforgedataset} & voice & 30 & >214 \\		
		\bottomrule
	\end{tabular}
	\caption{Datasets used for the analysis.}
	\label{tab:datasets}
\end{table}



==> sections/threatmodel.tex <==
\section{Threat Model}
\label{sec:threatmodel}


%Relate our stuff to this paper~\cite{Papernot2016}. 
%Then describe the objective, capabilities, and knowledge of the adversary~\cite{Biggio2017}.

The adversary's overarching goal is to place a ``biometric backdoor'' which grants him long-term access to the secured system without requiring further effort once the backdoor is in place. In this section, we define the attacker's objectives, knowledge and capabilities.
%While a variety of attacks on biometric authentication have been proposed in literature, they typically require significant cognitive effort and come with the risk of detection. 

\myparagraph{Objectives}
The attacker's goals are to:
\begin{itemize}[leftmargin=0.5cm]
	\item Cause modifications of the user template that leads to the attacker being accepted.
	\item Avoid alerting the user by compromising error rates (i.e., minimal changes to FRR and FAR).
	\item Minimize the number of physical accesses to the system required to plant the backdoor.
	\item Minimize the number of samples rejected by the recognition system.
	
\end{itemize}

\begin{figure}[t]
	\includegraphics[width=0.48\textwidth]{images/threat-model}
	\caption{Threat model. Both adversaries alter the biometric template before it reaches the application environment.}
	\label{fig:threat-model}
\end{figure}


\myparagraph{Capabilities}
\todo{n of query argument and failures argument}
We assume that the adversary can alter biometric sensor measurements to some degree.
This assumption follows from the extensive research on attacks against biometric authentication presented in Section~\ref{sec:relatedwork}.
We discriminate between two types of adversaries based on their capabilities, shown in Figure~\ref{fig:threat-model}:
\begin{itemize}[leftmargin=0.5cm]
	\item \textit{Complete input manipulation} -- the adversary has direct (automatable) access to the biometric sensor and can therefore freely inject arbitrary samples. As a result, the injected samples can be chosen with perfect accuracy and zero noise.
	\item \textit{Physical input manipulation} -- the adversary has physical access to the sensor and is able to feed samples to it. 
	As a result, the attacker is unable to reproduce the entire feature space and individual samples are subject to both sensor and presentation noise.

\end{itemize}

We assume both adversaries alter the biometric measurement before it reaches the protected application environment.
Differently from related works, we do \textbf{not} assume that the attacker has access to the system during enrolment or during any subsequent replacements of the complete template.
The adversary is also unable to directly change the template or training data (e.g., by removing or replacing user samples).

\myparagraph{Knowledge}
The adversary's knowledge can be split into two components: knowledge of the victim's template and knowledge of the system.
We assume that the adversary has at least some knowledge about the victim's biometric trait.
%(but does not necessarily possess any of the training samples that make up the template).
This is in line with assumptions made in related work (see Section~\ref{sec:relatedwork}).
Being a physiological feature, face geometry is notoriously difficult to keep secret. Social media in particular is a plentiful source for photographs from different angles.
Speaker recognition suffers from a similar problem, with adversaries being able to record the victim's voice during daily interactions.
We also assume that the attacker knows the details of the recognition algorithm.
This includes the features, the ML model(s) and the matching technique used in the recognition pipeline.
%The reasoning for this is that regardless of the specific feature definition and classifier used, the underlying \textit{identifying information} is the same.
%This intuition is supported by successful attacks on biometric recognition systems without any knowledge of the features (see, e.g.,~\cite{eberz2017broken}).
With the wide-spread use of DNN for biometric recognition, the features tend to be the exact raw biometric measurements, whose format is known (e.g., pixels for face recognition).
As such, the proposed attack will not be specific to individual features.
However, regarding the knowledge of the victim's template, we define two types of attackers as follows:

\begin{itemize}[leftmargin=0.5cm]
	\item \textit{Full knowledge} -- the attacker knows the enrolled user template (the training samples) as well as the template update procedure. As a result, he can calculate the precise location of decision boundaries. As he knows the matching procedure and parameters, he can also predict the effects of template updates (i.e., addition of training samples to the template and resulting boundary changes).
	\item \textit{Minimal knowledge} -- the attacker only knows  one user sample that is accepted by the system (e.g., by observation, collection or guessing). He does not know the enrolled user template or the resulting decision boundaries. In addition, he does not know if and how the training set and decision boundaries are altered after template updates.
\end{itemize}

Based on these two dimensions (knowledge and capabilities), we define two types of attackers: \textit{Perfect} and \textit{weak} attackers:
\begin{itemize}[leftmargin=0.5cm]
	\item \textbf{Perfect} attackers have complete knowledge of the system and user (i.e., the full knowledge model described above). In addition, they are capable of complete input manipulation.
	\item \textbf{Weak} attackers are only capable of physical input manipulation. As a result, their reproductions of input samples will be subject to noise.
	Similarly to perfect attackers, weak attackers also know the models and algorithms used in the recognition.
	However, they don't have knowledge of neither the template nor how it is affected by any updates (i.e., the minimal knowledge model described above).
\end{itemize}

Throughout the paper, we use the perfect attacker as a mean to establish best-case upper bounds for the poisoning attack's effectiveness.
%In addition, we use population data from the perfect attacker model as a basis for the weak attacker model's predictive heuristic (see Section~\ref{sec:attackdesign}).
The final results will be based on the weak attacker, which is a much more realistic threat model in practice.

